How quantum selection rules influence the magneto-optical effects of driven, ultrafast magnetization dynamics

Ultrafast magnetization dynamics driven by ultrashort pump lasers is typically explained by changes in electronic populations and scattering pathways of excited conduction electrons. This conventional approach overlooks the fundamental role of quantum mechanical selection rules, governing transitions from core states to the conduction band, that forms the key method of the probing step in these experiments. By employing fully ab initio time-dependent density functional theory, we reveal that these selection rules profoundly influence the interpretation of ultrafast spin dynamics at specific probe energies. Our analysis for hcp Co and fcc Ni at the M edge demonstrates that the transient dynamics, as revealed in pump-probe experiments, arise from a complex interplay of optical excitations of the M shell. Taking into account the selection rules and conduction electron spin flips, this leads to highly energy-dependent dynamics. These findings address longstanding discrepancies in experimental TMOKE measurements and show that only through meticulous consideration of matrix elements at the probe stage, can one ensure that magnetization dynamics is revealed in its true nature, instead of being muddled by artifacts arising from the choice of probe energy.

==> backups/main-241008.tex <==
An Ab Initio Investigation of the Interplay of Optics, Magnetism, and Quantum
Mechanics in Ultrafast Magnetization Dynamics
Mohamed F. Elhanoty,1, ∗ Olle Eriksson,1, 2 Chin Shen Ong,1 and Oscar Gr˚an¨as1, †
1Division of Materials Theory, Department of Physics and Astronomy,
Uppsala University, Box-516, SE 75120, Sweden
2Wallenberg Initiative Materials Science for Sustainability (WISE), Uppsala University, 75121 Uppsala, Sweden
(Dated: October 8, 2024)
Ultrafast magnetization dynamics driven by ultrashort pump lasers is traditionally studied
through changes in electronic populations and scattering pathways of excited conduction electrons.
Yet, this conventional approach neglects the fundamental role of quantum mechanical selection
rules governing transitions from core states to the conduction band. By employing the fully ab ini-
tio time-dependent density functional theory, we reveal the profound impact of the selection rules
on the observed ultrafast spin dynamics at specific energies. Our analysis of hcp Co and fcc Ni at
the M edge shows that the transient dynamics in pump-probe experiments arise from a complex
interplay of optical excitations, conduction electron spin flips, and selection rules, leading to highly
energy-dependent dynamics. Our analysis is important for resolving discrepancies in the measured
T-MOKE signals and emphasizes the importance of meticulousness in interpreting the transient
dynamics, ensuring that the pump-induced dynamics are distinguished from artifacts arising from
the choice of probe energy.
INTRODUCTION
As we advance toward the next generation of ultrafast
and highly efficient devices, the challenge of developing
magnetic data storage solutions that can meet the grow-
ing demands for speed and reliability becomes increas-
ingly critical [1–3]. Leveraging ultrafast magnetization
dynamics through the use of ultrashort laser pulses of-
fers a promising approach to revolutionize magnetic data
storage. This method has the potential to enable un-
precedented data transfer rates and storage densities by
manipulating magnetic states with unmatched precision
and speed [1, 4]. However, uncovering the ultrafast re-
sponse of magnetic materials to femtosecond laser pulses
presents a complex challenge due to the involvement of
multiple degrees of freedom, each interacting on different
timescales [5–7].
The pump laser couples directly to the valence and
conduction electrons of the material, leading to demag-
netization [4, 6]. In Ref. [8], three key microscopic pro-
cesses occurring within the first 100 fs are experimentally
and theoretically identified: spin flips mediated by spin-
orbit coupling (SOC), intrasite spin transfer within the
same species, and intersite spin transfer in multicompo-
nent magnetic alloys. Probing these ultrafast processes
at such short timescales is highly challenging and requires
measurement of the dynamics using probe energies reso-
nant with the excitation of core electrons to unoccupied
states in the conduction band [9].
Time-resolved pump-probe experiments, such as
transient transverse magneto-optical Kerr effect (TR-
TMOKE), have become essential tools for exploring ul-
trafast magnetization dynamics in both simple elements
and magnetic alloys, offering attosecond and femtosec-
ond time resolution [8–12]. In these experiments, a pump
laser excites the electronic system, and after a controlled
delay, a probe pulse captures the resulting dynamics. For
3d transition metals, T-MOKE measurements typically
use photon energies resonant with the 3p to 3d transi-
tions at the M-edge [13].
The SOC splits the 3p core levels into 3p3/2 and 3p1/2
states, resulting in distinct M3 and M2 absorption edges,
see Fig. 1 [14]. The energy difference between these lev-
els, typically 1–3 eV in transition metals, leads to a par-
tial overlap of the M3 and M2 edges as shown in Fig. 1 (b
and c) [14]. This overlap mixes their positive and nega-
tive contributions, complicating the interpretation of ex-
perimental signals and potentially leading to conflicting
measurements. This issue is central to the analysis pre-
sented in this work.
Recent investigations into the instantaneous magneti-
zation of different elements across varying probe energies
have revealed a highly debated energy-dependent ultra-
fast response [8, 15–17]. Three notable studies on Ni ob-
served stark contrasts within the first 100 fs, with certain
probe energies showing a reduction in intensity, while
other probe energies showed enhancement in the tran-
sient signal [15–17]. In another finding, measurements of
the transient MOKE signal revealed varying rates and in-
tensities of optical intersite spin transfer (OISTR) in the
Heusler compound Co2MnGa, depending on the probe
energy used [8]. These recent findings raise pivotal ques-
tions about the role of probe energy in the underlying
dynamics and whether the observed induced dynamics
result solely from the pump laser or from the interaction
of the optical probe with core electrons, as dictated by
quantum mechanical selection rules. Another fundamen-
tal question is whether microscopic processes induced by
a pump laser, such as optical excitation and spin flips,
would manifest unique signatures regardless of the probe
2
FIG. 1. (a) Schematic diagram illustrating the probe optical excitations and the spliting of the core states. The upper panel
displays the projected density of states (PDOS) for Ni and Co, where the shaded gray area below the Fermi level represents
the ground-state static occupation, and the unshaded region shows the empty states above the Fermi energy. The splitting of
the 3p core states into 3p3/2 and 3p1/2 sublevels, due to spin-orbit coupling (SOC), is shown, with the associated mj quantum
numbers in the lower panel. The probe laser excites electrons from the 3p core states to unoccupied states above the Fermi
level, EF. (b,c) The real part of the off-diagonal component of the dielectric tensor in the ground state, depicting the total M
edge along with contributions from the 3p3/2 (M3) and 3p1/2 (M2) states for Ni (top right panel) and Co (bottom right panel).
energy.
Here, we address these questions and challenges
through a detailed analysis of the static and transient di-
electric tensor of two Stoner magnets, hcp Co and fcc Ni,
at the M-edge, using the fully ab initio time-dependent
density functional theory (TD-DFT). We find that the
dynamics induced by the pump laser, including optical
excitation and spin flips, do not manifest unique sig-
natures in the transient dielectric tensor and vary with
the measuring energy. To identify the microscopic ori-
gins of these energy-dependent dynamics, we disentangle
the contributions of each core state within the 3p3/2 and
3p1/2 manifolds to the total static and transient signals
of the M3 and M2 edges respectively. We find that the
constituent states of the M3 and M2 edges have different
optical response to the induced dynamics by the pump
laser and the superposition of their contribution to the
optical response lead to highly energy dependent dynam-
ics. Our findings indicate that the observed variations in
energy-dependent dynamics, reported in recent ultrafast
experiments [8, 15, 16], arise from a complex interplay
of optical excitations, conduction electron spin flips, and
selection rules that depend on the availability of states
for optical transitions and the spin character of the initial
and final states.
RESULTS
The magnetization is related to dielectric tensor ac-
cording to the following equation [18]:
M ∝ ℜ{ ϵxy sin 2θi
n4 cos2 θi − n2 + sin2 θi
} (1)
where θi and θt are the incident and the transmission an-
gles respectively and n is the refractive index. To make
our discussion free of the complications of the experimen-
tal geometry of the Fresnel equation [17], we focus in our
discussion on the off diagonal component of the dielectric
tensor ϵxy . For more details, see the methods section.
Fig. 2 illustrates the variation in the real components
of ℜϵxy at 35 fs, relative to the ground-state values pre-
sented in Fig. 1. For the total M edge data, where the
edges M3 and M2 overlap in Fig. 2 (a and c), the energy-
dependent dynamics are highly pronounced. Within the
energy range of 60 to 65 eV for Ni and 55 to 60 eV for Co,
the transient changes exhibit distinct behavior, with the
dynamics changing sign beyond 65 eV for Ni and 60 eV
for Co, showing more pronounced oscillatory patterns.
To quantify the effect of edge overlap on these energy-
dependent dynamics, we deconvolve the contributions of
the individual M3 and M2 edges in Fig. 2 (b and d). In
the 60 to 65 eV range for Ni and 55 to 60 eV for Co, the
M2 edge contribution is minimal and retains the same
3
FIG. 2. (a, c) The changes in the real part of the off-
diagonal component of the dielectric tensor at 35 fs relative
to the ground state for the total M-edge for Ni in (a) and Co
in (c). (b, d) The changes in the 3p3/2 (M3) and 3p1/2 (M2)
states for Ni in (b) and Co in (d).
negative sign as the M3 edge changes. However, beyond
the resonance threshold (greater than 65 eV for Ni and
60 eV for Co), the M3 and M2 edges exhibit alternating
dynamics. Importantly, in this region, both static and
transient behavior are strongly influenced by the signifi-
cant overlap between the M3 and M2 edges.
Interestingly, the magnetic moment of hcp Co de-
creases from 3.11 μB to 2.84 μB and fcc Ni from 0.61 μB
to 0.58 μB due to spin flips mediated by the SOC. A fun-
damental question arises: Why is this change in magnetic
moment accompanied by such highly energy-dependent,
and even contradictory, dynamics between the M3 and
M2 edges? To address this question, we decompose the
static and transient contributions in Fig. 3 and Fig. 5,
isolating the contributions from each core state of the
3p3/2 and 3p1/2 manifolds to the total intensity of the M3
and M2 edges, respectively. This detailed breakdown of-
fers critical insight into the role of individual core states
in driving the complex energy-dependent behavior ob-
served.
In atomic systems, the choice between Russell-
Saunders coupling (LS) and jj coupling depends on the
competition between the SOC and electrostatic interac-
tions [19, 20]. For valence electrons in lighter atoms, the
LS coupling is more suitable due to weaker SOC [21].
However, for core electrons, where SOC is stronger, the
jj coupling scheme becomes more appropriate and pro-
vides a more diagonal representation [21]. The presence
of relatively stronger SOC for the core states leads to
mixing the spin up and spin down components. In ad-
dition, the spin angular momentum is no longer a good
quantum number due to SOC. The mixing of spin compo-
nents in the core states plays a key role in explaining the
FIG. 3. Decomposition of the total M3 and M2 edges for Ni,
shown in panels (a) and (b), and Co, shown in panels (c) and
(d) into their constituent 3p3/2 and 3p1/2 components. For
Ni, the 3p3/2 states are represented by mj= 3
2
= − 3
2 , − 1
2 , 1
2 , 3
2 ,
and the 3p1/2 states are represented by mj= 1
2
= − 1
2 , 1
2 . For
Co, the 3p3/2 and 3p1/2 components are similarly identified in
panels (c) and (d). The colors for the states follow the same
list in schematic of Fig. 1.
energy dependence of both static and transient signals as
discussed in detail below.
The intensity at a given M3 edge energy is a su-
perposition of contributions from the states mj= 3
2 =
{− 3
2 , − 1
2 , 1
2 , 3
2 }, while the probe signal resonating with
the M2 edge is a superposition of states mj= 1
2 = {− 1
2 , 1
2 }.
The transition probabilities between these core states
and the empty conduction band states are governed by
Clebsch-Gordan coefficients, which result from the cou-
pling between spin and orbital angular momenta [22].
These coefficients determine the relative weights of the
different mj states in the final optical spectra, leading to
unequal contributions from each core state.
A detailed examination of the 3p3/2 manifold contri-
butions for both Co and Ni, shown in Fig. 3 (a and c),
reveals that the mj = − 1
2 state contributes a signifi-
cant positive component, while the mj = − 3
2 state pro-
vides a significantly larger negative component, resulting
in an overall net negative contribution at the M3 edge.
The contributions from the other states, mj = 1
2 and
mj = 3
2 , are relatively small and nearly cancel out each
other. Thus, for the purposes of the discussion, these
states can be disregarded.
For the 3p1/2 manifold, as shown in Fig. 3 (b and d),
the mj = 1
2 state gives a small negative contribution,
whereas the mj = − 1
2 state contributes a larger positive
component, leading to a net positive signal at the M2
edge. Notably, the contributions from each core state of
the 3p3/2 and 3p1/2 manifolds to the M3 and M2 edges,
4
respectively, are overlapping, as demonstrated in Fig. 3.
To elucidate the impact of the spin mixing in the core
states on both static and transient signals, Fig. 4 illus-
trates the relative weights of their bands in the spin-up
and spin-down projections. The 3p1/2 and 3p3/2 states of
FIG. 4. Spin-up and spin-down projections of the ground
state band structure for the 3p states. Panels (a) and (b)
depict the spin-up and spin-down projections for Ni, respec-
tively, and panels (c) and (d) show the corresponding projec-
tions for Co.
Co and Ni consist of four (two) and eight (four) states, re-
spectively, each exhibiting varying contributions of spin-
up and spin-down projections, as shown in Fig. 4. In
the 3p1/2 manifold, the state with mj = 1
2 for both el-
ements has its primary contribution from spin-up, while
the state with mj = − 1
2 has its main contribution from
spin-down. Given that most of the empty states above
the Fermi level, available for optical excitation, exhibit
spin-down character (see Fig. 1a), the optical transitions
with spin-down character contribute significantly to the
final signal, resulting in a more intense contribution from
the mj = − 1
2 state than the mj = 1
2 state, see Fig. 3b
and d.
Similarly, the mj = − 3
2 state is primarily composed of
spin-down contributions, while the mj = − 1
2 and mj = 1
2
states are mixtures of both spin-up and spin-down com-
ponents. Therefore, the mj = − 3
2 state manifests a
strong negative contribution, while the mj = − 1
2 and
mj = 1
2 states produce smaller positive contributions,
leading to a net overall negative contribution at the M3
edge, see Fig. 3 (a and c).
TRANSIENT DYNAMICS
Having identified the overlapping states of the M3 and
M2 edges and their distinct contributions to the overall
signal, a critical question arises: Do the ultrafast elec-
tron dynamics induced by the pump laser exhibit unique
signatures in the transient signals of each core state, or
does their different spin character determine the intensi-
ties of this response? Furthermore, it is crucial to assess
the impact of the superposition of the contributions from
each core state within the M3 and M2 manifolds. Specif-
ically, we must investigate whether the overlapping core
states with different signs, as analyzed in Fig. 3, compete
against each other, resulting in the alternating and even
contradictory dynamics presented in Fig. 2.
To elucidate the subtle variations in the magnitude of
the dielectric tensor, we separate the contributions in the
ground state (GS) and at 35 fs from the two predominant
states at the M3 edge (mj = − 3
2 and mj = − 1
2 ) and the
states at the M2 edge (mj = − 1
2 and mj = 1
2 ), as detailed
in Fig. 5.
FIG. 5. Separation of contributions to the dielectric tensor
at the M3 and M2 edges in the ground state (solid lines) and
at 35 fs (dashed lines). Panel (a) displays the mj = 3
2 and
mj = − 1
2 states in the 3p3/2 manifold, and panel (b) shows
the mj = 1
2 and mj = − 1
2 states in the 3p1/2 manifold for Ni
in the ground state and at 35 fs. Panels (c) and (d) show the
corresponding states for Co.
For the M3 edge of Ni and Co, as shown in Fig. 5 (a
and c), the magnitude of the contributions from both
mj = − 3
2 and mj = − 1
2 states is significantly reduced
due to spin-flip transitions and optical excitation. How-
ever, the intensity of the mj = − 1
2 state remains posi-
tive, while the intensity of the mj = − 3
2 state is negative.
Their overlap results in a partial cancellation of the in-
duced changes. This occurs because the mj = − 3
2 state
predominantly exhibits spin-down character, whereas the
mj = − 1
2 state exhibits a mixed spin-up and spin-down
character (see Fig. 4). Similarly, the overlap between the
5
mj = 1
2 and mj = − 1
2 states at the M2 edge reduces
the observable changes in charge and spin dynamics, see
Fig. 5b and d. Note that the 3p1/2 states has further over-
lap from the extended part of the 3p3/2 states (mj = − 3
2
and mj = − 1
2 ) states that extend to 70 eV for Ni and 65
eV for Co leading to further complication of interpreting
the signal measured at the M2 edge, see Fig. 5. There-
fore, interpreting the measurements probed at probing
energies resonating with the M2 is unreliable due to the
superposition of various contributions.
DISCUSSION AND CONCLUSION
A key unresolved question in the field of ultrafast mag-
netization dynamics is whether the asymmetry observed
in time-resolved magneto-optical Kerr effect (T-MOKE)
experiments directly correlates with changes in magneti-
zation. The interpretation of distinct dynamics at differ-
ent probing energies has also been a topic of considerable
debate. Our study provides significant insights into the
complex relationship between spin-orbit coupling (SOC)
and ultrafast electron dynamics.
The SOC in conduction electrons predominantly en-
ables spin flips, whereas in core states, it mixes the spin-
up and spin-down components but also induces an en-
ergy splitting of 1–3 eV between the 3p3/2 and 3p1/2
states [23–25]. This leads to a partial overlap between
the M3 and M2 edges and plays a fundamental role in
shaping the observable optical transitions. Our resolu-
tion of the individual contributions from the 3p3/2 and
3p1/2 states to the dielectric tensor at the M3 and M2
edges highlights the nuanced impact of this spin mixing
on ultrafast magnetization dynamics.
In addition to spin flips, pump lasers drive optical exci-
tations of electrons from occupied states below the Fermi
level to unoccupied states above it, resulting in the for-
mation of holes below the Fermi level and the popula-
tion of states above it [8]. Although charge excitations
within the same spin channel preserve total spin, they
leave distinct signatures in the dielectric tensor. These
signatures are influenced by quantum mechanical selec-
tion rules, electron occupation, and the spin character of
both the initial core state and the final conduction state.
The role of Clebsch-Gordan coefficients in modulat-
ing relative transition probabilities highlights the impor-
tance of rigorously applying quantum mechanical selec-
tion rules in the analysis of energy-dependent ultrafast
magnetization dynamics. Ultrafast processes, including
optical excitations and spin-flip mechanisms, result in a
reduction in magnetic moment, which is reflected in the
transient dielectric tensor, especially at the M3 and M2
absorption edges. The partial spectral overlap of these
edges complicates interpretation, as changes at one edge
inevitably influence the observed dynamics at the other.
Specifically, the mj = − 3
2 and mj = − 1
2 states at the M3
edge overlap with the mj = − 1
2 and mj = 1
2 states at the
M2 edge. The contributions from these states partially
counteract each other, leading to a subtle net observable
effect. Disentangling individual core-state contributions
at both edges is crucial for fully understanding the com-
plex superposition of effects within the measured signal.
To improve the interpretation of transient signals, we
recommend three critical steps: (1) a comprehensive as-
sessment of the overlap between the M3 and M2 edges,
(2) the resolution of contributions from each core state,
with careful attention to the character of their spin pro-
jection, and (3) conducting time-resolved (T-MOKE) ex-
periments at multiple probing energies, specifically in re-
gions without spectral overlap. This is especially impor-
tant for multicomponent alloys, where optical intersite
spin transfer is anticipated [8]. Based on our analysis of
Co and Ni, we suggest focusing measurements on the M3
edge to yield more reliable results.
Our quantum mechanical approach here, based on se-
lection rules, provides a robust framework for disentan-
gling contributions from overlapping M3 and M2 edges.
This approach enables us to resolve the superposition of
core states with differing spin characteristics paving the
way for more accurate predictions and control over ma-
terial properties on the femtosecond timescale.
METHODS
TDDFT
Through the one to one mapping between the time
dependent density n(r, t) and the external potential
Vext(r, t), Runge and Gross extended the ab initio
ground state Kohn Sham density functional theory to
the time domain [26]. This mapping allows for a fully
interacting system to be represented by an equivalent
non-interacting one with a time dependent Kohn-Sham
(KS) effective potential vs(r,t), that produces the same
density as the fully interacting system. The KS effec-
tive potential, vs(r, t), is a sum of three terms vs(r, t) =
vext(r, t) + vH(r, t) + vxc(r, t), where vext(r, t) is the ex-
ternal potential, vH(r, t) is the Hartree potential, and
vxc(r, t) is the exchange-correlation (XC) potential. The
TDKS can be written as:
 1
2
 − i∇ + 1
c Aext(t)2 + vs(r, t) + 1
2c σ · Bs(r, t)+
1
4c2 σ · ∇vs(r, t) × −i∇
ψi(r, t) = ∂ψi(r, t)
∂t ,
(2)
where c is the speed of light, σ is the Pauli matrix, and
Bs(r, t) is the effective KS magnetic field (Bs(r, t) =
Bext(t) + Bxc(r, t), where Bext(t) is the magnetic field
of the external laser pulse and Bxc(r, t) is the xc induced
exchange splitting. The last term in Eq. 2 is the SOC
6
term and ψi(r, t) is two component Pauli spinor. If the
material is driven out of equilibrium by an external laser,
the dipole approximation for the vector potential Aext(t)
of the pump laser is usually used for wavelengths much
larger than the lattice constant. The atomic units (with
ℏ = e =m=1) are adopted in Eq. 2.
Linear response
The mixed scheme between the time evolution of Eq. 2
and the linear response introduced by Dewhurst et al, [27]
is employed but with some modifications presented in
Ref. [8, 28] to calculate the response function at a 45 fs
time. The non interacting (KS) response function can be
written as [29]:
χs(r, r′
, ω) = lim
η→0
∞X
i=1
∞X
j=1
(ni−nj ) ψ∗
i (r)ψj (r)ψi(r′
)ψ∗
j (r′
)
ω − ϵj + ϵi + iη
(3)
where ψi is the KS orbital, ϵi their eigenvalues, and ni
the occupation number.
The interacting response function, χ, is related to the
non interacting one, χs through the following Dyson
equation:
χ(r, r′
, ω) = χs(r, r′
, ω)+χs(r, r′
, ω)(ν+fxc(ω))χ(r, r′
, ω)
(4)
where ν is the is the bare Coulomb interaction and
fXC is the exchange-correlation kernel. The dielectric
tensor,ϵ(ω), is calculated using the response function ac-
cording to the following equation [30]:
ϵ−1
ij (ω) = δij + νχij (ω) (5)
Numerical Details
The time evolution of Eq. 2 and the linear response
calculation are performed using the full potential basis
ELK code [31]. The FWHM of the pump laser is 35 fs,
with energy 1.55 eV corresponding to wavelength of 800
nm and a fluence of 12 mj/cm2. The time step of the
time evolution is 2.4 as. The transient linear response
calculations were performed as detailed in Ref. [8, 28]
ACKNOWLEDGEMENTS
The computations were enabled by resources provided
by the Swedish National Infrastructure for Computing
(SNIC) at NSC and Uppmax partially funded by the
Swedish Research Council through grant agreement no.
2018-05973. OG acknowledge financial support from the
Strategic Research Council (SSF) grant ICA16-0037 and
the Swedish Research Council (VR) grant 2019-03901.
This work was also supported by the European Research
Council via Synergy Grant 854843 - FASTCORR.
∗ mohamed.elhanoty@physics.uu.se
† Corresponding Author: oscar.granas@physics.uu.se
[1] B. Bhushan, Microsystem Technologies 29, 1529 (2023).
[2] B. Dieny, I. L. Prejbeanu, K. Garello, P. Gambardella,
P. Freitas, R. Lehndorff, W. Raberg, U. Ebels, S. O.
Demokritov, J. Akerman, et al., Nature Electronics 3,
446 (2020).
[3] A. Hirohata, K. Yamada, Y. Nakatani, I.-L. Prejbeanu,
B. Di´eny, P. Pirro, and B. Hillebrands, Journal of Mag-
netism and Magnetic Materials 509, 166711 (2020).
[4] A. Kimel, A. Zvezdin, S. Sharma, S. Shallcross,
N. De Sousa, A. Garc´ıa-Mart´ın, G. Salvan, J. Hamrle,
O. Stejskal, J. McCord, et al., Journal of Physics D: Ap-
plied Physics 55, 463003 (2022).
[5] M. Shirozhan, S. Mondal, T. Gr´osz, B. Nagyill´es,
B. Farkas, A. Nayak, N. Ahmed, I. Dey, S. C. De Marco,
K. Nelissen, et al., Ultrafast Science 4, 0067 (2024).
[6] A. Kirilyuk, A. V. Kimel, and T. Rasing, Reviews of
Modern Physics 82, 2731 (2010).
[7] C. Wang and Y. Liu, Nano Convergence 7, 1 (2020).
[8] S. A. Ryan, P. C. Johnsen, M. F. Elhanoty, A. Grafov,
N. Li, A. Delin, A. Markou, E. Lesne, C. Felser, O. Eriks-
son, et al., Science Advances 9, eadi1428 (2023).
[9] B. Buades, A. Pic´on, E. Berger, I. Le´on, N. Di Palo, S. L.
Cousin, C. Cocchi, E. Pellegrin, J. H. Martin, S. Ma˜nas-
Valero, et al., Applied Physics Reviews 8 (2021).
[10] C. La-O-Vorakiat, M. Siemens, M. M. Murnane, H. C.
Kapteyn, S. Mathias, M. Aeschlimann, P. Grychtol,
R. Adam, C. M. Schneider, J. M. Shaw, et al., Physi-
cal Review Letters 103, 257402 (2009).
[11] B. Vodungbo, J. Gautier, G. Lambert, A. B. Sardinha,
M. Lozano, S. Sebban, M. Ducousso, W. Boutu, K. Li,
B. Tudu, et al., Nature communications 3, 999 (2012).
[12] P. Tengdin, C. Gentry, A. Blonsky, D. Zusin, M. Gerrity,
L. Hellbr¨uck, M. Hofherr, J. Shaw, Y. Kvashnin, E. K.
Delczeg-Czirjak, et al., Science advances 6, eaaz1100
(2020).
[13] C. La-o vorakiat, Ph. D. Thesis (2011).
[14] F. De Groot and A. Kotani, Core level spectroscopy of
solids (CRC press, 2008).
[15] M. Hennes, B. R¨osner, V. Chardonnet, G. S. Chiuzba-
ian, R. Delaunay, F. D¨oring, V. A. Guzenko, M. Hehn,
R. Jarrier, A. Kleibert, et al., Applied Sciences 11, 325
(2020).
[16] H.-T. Chang, A. Guggenmos, S. K. Cushing, Y. Cui,
N. U. Din, S. R. Acharya, I. J. Molesky, U. Kleineberg,
V. Turkowski, T. S. Rahman, et al., Physical Review B
103, 064305 (2021).
[17] H. Probst, C. M¨oller, M. Schumacher, T. Brede, J. K. De-
whurst, M. Reutzel, D. Steil, S. Sharma, G. S. M. Jansen,
and S. Mathias, Phys. Rev. Res. 6, 013107 (2024).
[18] P. M. Oppeneer and A. Liebsch, Journal of Physics: Con-
densed Matter 16, 5519 (2004).
[19] E. U. Condon and G. H. Shortley, The theory of atomic
spectra (Cambridge University Press, 1935).
[20] H. A. Bethe and E. E. Salpeter, Quantum mechanics of
one-and two-electron atoms (Springer Science & Business
7
Media, 2013).
[21] B. H. Bransden and C. J. Joachain, Physics of atoms and
molecules (Pearson Education India, 2003).
[22] J. St¨ohr and H. C. Siegmann, Solid-State Sciences.
Springer, Berlin, Heidelberg 5, 236 (2006).
[23] I. ˇZuti´c, J. Fabian, and S. D. Sarma, Reviews of modern
physics 76, 323 (2004).
[24] B. Thole and G. Van der Laan, Physical Review B 38,
3158 (1988).
[25] G. Van der Laan and I. Kirkman, Journal of Physics:
Condensed Matter 4, 4189 (1992).
[26] E. Runge and E. K. Gross, Physical review letters 52,
997 (1984).
[27] J. Dewhurst, F. Willems, P. Elliott, Q. Li, C. v. K.
Schmising, C. Str¨uber, D. Engel, S. Eisebitt, and
S. Sharma, Physical Review Letters 124, 077203 (2020).
[28] T. Lojewski, M. F. Elhanoty, L. Le Guyader, O. Gr˚an¨as,
N. Agarwal, C. Boeglin, R. Carley, A. Castoldi, C. David,
C. Deiter, et al., Materials Research Letters 11, 655
(2023).
[29] M. Petersilka, U. Gossmann, and E. Gross, Physical re-
view letters 76, 1212 (1996).
[30] P. Oppeneer, T. Maurer, J. Sticht, and J. K¨ubler, Phys-
ical Review B 45, 10924 (1992).
[31] “The Elk Code,” http://elk.sourceforge.net/.
